Joint Object Contour Points and Semantics for Instance Segmentation

The attributes of object contours has great significance for instance segmentation task. However, most of the current popular deep neural networks do not pay much attention to the object edge information. Inspired by the human annotation process when making instance segmentation datasets, in this paper, we propose Mask Point R-CNN aiming at promoting the neural network's attention to the object boundary. Specifically, we innovatively extend the original human keypoint detection task to the contour point detection of any object. Based on this analogy, we present an contour point detection auxiliary task to Mask R-CNN, which can boost the gradient flow between different tasks by effectively using feature fusion strategies and multi-task joint training. As a consequence, the model will be more sensitive to the edges of the object and can capture more geometric features. Quantitatively, the experimental results show that our approach outperforms vanilla Mask R-CNN by 3.8\% on Cityscapes dataset and 0.8\% on COCO dataset.

==> Permutation.tex <==
\section{Designing parallel permutation}
\label{sec2}
This section is organized as follows: discuss the original motivation to design this algorithm;
explain how our permutation works;
elaborate on the entire permutation process.

An image with a gray-scale of $256$ can be considered as a set of eight bit planes.  
\begin{figure}[htbp]
	\centering
	\mbox{
		\subfigure[$1^{st}$bit plane]{\includegraphics [width=0.2\linewidth]{permutationimg/Lena_bin0.jpg}}
		\subfigure[$2^{nd}$bit plane]{\includegraphics [width=0.2\linewidth]{permutationimg/Lena_bin1.jpg}}
		\subfigure[$3^{rd}$bit plane]{\includegraphics [width=0.2\linewidth]{permutationimg/Lena_bin2.jpg}}
		\subfigure[$4^{th}$bit plane]{\includegraphics [width=0.2\linewidth]{permutationimg/Lena_bin3.jpg}}
	}
	\mbox{
		\subfigure[$5^{th}$bit plane]{\includegraphics [width=0.2\linewidth]{permutationimg/Lena_bin4.jpg}}
		\subfigure[$6^{th}$bit plane]{\includegraphics [width=0.2\linewidth]{permutationimg/Lena_bin5.jpg}}
		\subfigure[$7^{th}$bit plane]{\includegraphics [width=0.2\linewidth]{permutationimg/Lena_bin6.jpg}}
		\subfigure[$8^{th}$bit plane]{\includegraphics [width=0.2\linewidth]{permutationimg/Lena_bin7.jpg}}
	}
	\caption{The binary images of eight bit planes.}
	\label{bin8img}
\end{figure}
A pixel value $\mathit{Pv}$ is represented by,
\begin{equation}
\label{eq1}
Pv = \sum_{i = 0}^{7}2^i\times bp_i,
\end{equation}
where $\mathit{bp_{i}}\in\{0, 1\}$.
From the Eq.(\ref{eq1}), it can be calculated that the higher four bit planes have $94.1\%$ information of an image.  
It means that the higher four bit planes have more impact on human visual system than lower four bit planes. 
It is seen as an intrinsic feature of the bit distribution of images in~\cite{zhang2013symmetric}.
Fig.~\ref{bin8img} shows the Lena image in eight bit planes.
It can be seen that the higher bit planes contain the majority of the visually significant data, 
and the lower four bit planes act as random noises.
%It's also considered as an intrinsic feature of different bit planes. 
These intrinsic features of bit distribution inspire us to randomly put lower bit planes in the higher position to hide plaintext information.
Besides the features mentioned above, most bits at the same position in $7$th and $8$th bit planes have opposite values, 
showing that the two bit planes have a strong correlation~\cite{zhang2013symmetric}.
Therefore, we exchange bits of higher bit planes with lower bit planes to remove the correlation between higher bit planes.
%So this intrinsic feature inspires us that we can randomly put the bit planes in the lower position to the higher position to hide plaintext information.  
In our proposed parallel bit-level permutation algorithm, eight bit planes are randomly divided into four groups, 
and two bit planes in each group exchange bits with each other.
The operations in four groups are executed in a parallel manner. 
There are no data disorder problems when multiple threads work concurrently because the behavior of exchanging bits in each group does not affect each other.
%and the experimental results show that our parallel bit-level method is efficient and has a good permutation effect. 

\subsection{Grouping bit planes with logistic map} 
\label{sub2.1}
Our parallel bit-level permutation operation consists of two different stages. 
In the first round, we divide the eight bit planes into two sets.
One consists of the higher four bit planes, and the other consists of the lower four bit planes.
To hiding plaintext information, we only allow the exchange of bits between two groups from different sets.
Fig.~\ref{1stper} shows an example of the first round of permutation.
\begin{figure}
	\centerline{\includegraphics[width = 0.7\textwidth]{permutationimg/bperm.jpg}}  \caption{The
		first round of permutation.}\label{1stper}
\end{figure}%后面的描述我要跟着这个框架图走啊
In this example, the combination of different bit planes is $[(\mathit{bp}_7\leftrightarrow \mathit{bp}_1), (\mathit{bp}_6\leftrightarrow \mathit{bp}_0), (\mathit{bp}_5\leftrightarrow \mathit{bp}_3),(\mathit{bp}_4\leftrightarrow \mathit{bp}_2)]$. 
After the first round of permutation, the higher bit planes and lower bit planes have merged into each other,
and the statistical information of plain-image has been successfully masked.
Therefore in the following rounds, any two bit planes are grouped together repeatedly.


We employ the chaotic logistic map~\cite{matthews1989derivation} to assign the eight bit planes into four groups randomly.
Mathematically, the map is defined by,
\begin{equation}
\label{eqlogistic}
x_{n+1} = \mu x_{n}(1 - x_{n}),
\end{equation}
where $\mathit{\mu}\in(0, 4]$ is the control parameter.
The value of $\mathit{\mu}$ is set to $4$ for the best chaotic behavior.  
Fig.~\ref{logistic} shows its bifurcation diagram. 
\begin{figure}[]
	\centerline{\includegraphics[width = 0.6\textwidth]{permutationimg/logistic.jpg}} \caption{The bifurcation 
		diagram of logistic map.}\label{logistic}
\end{figure}

The detailed procedure for grouping bit planes is depicted in Alg.~\ref{secbp}.
Here $\mathit{lgInit_{bpgrp}}$ represents the initial values of the logistic map (\ie $\,$ $x_0$) used in bit plane grouping, 
while $\mathit{permRnd}$ represents the current permutation round. 
An array $\mathit{bps} = \{0, 1, 2, 3 , 4, 5, 6, 7\}$ represents identifiers of eight bit planes.
$\mathit{numUnselBp}$ represents the number of the unselected bit planes, and its initial value is $8$. 
$\mathit{hnumNunsecbp}$ represents half of $\mathit{numUnselBp}$, and its initial value is $4$. 
After selecting two bit planes, the value of $\mathit{numUnselBp}$ is decreased by $2$ and the value of $\mathit{hnumUnselBp}$ is decreased by $1$.
$\mathit{bp}1$ and $\mathit{bp}2$ represent the two selected bit planes.
\begin{algorithm}[]  
	\caption{The random grouping of bit planes.}  
	\label{secbp}  
	\begin{algorithmic}[1]  
		\Require  
		$\mathit{lgInit_{bpgrp}}, \mathit{permRnd}, \mathit{bps}, \mathit{hnumUnselBp}, \mathit{numUnselBp}$
		\Ensure  
		$\mathit{bp}1, \mathit{bp}2$
		\Function{bpGrp}{$\mathit{lgInit_{bpgrp}}, \mathit{permRnd}, \mathit{bp}, \mathit{hnumUnselBp}, \mathit{numUnselBp}$}
		\State $x_0 \gets \mathit{lgInit_{bpgrp}}$ and pre-iterate logistic map for $\mathit{T}_0$ times 
		\State Iterate logistc map for two times $\to$ $\mathit{x}_1, \mathit{x}_2$
		\If{$\mathit{permRnd} == 0$}
		\State $\mathit{bp}1 = \mathit{bp}[(int64)(\mathit{x}_{1}\times 10^{15})\mod \mathit{hnumUnselBp}]$
		\State Swap the values between $\mathit{bp}1$ and $\mathit{bp}[hnumUnselBp-1]$
		\State $\mathit{bp}2 = \mathit{bp}[4+(int64)(\mathit{x}_{2}\times 10^{15})\mod\mathit{hnumUnselBp}]$
		\State Swap the values between $\mathit{bp}2$ and $\mathit{bp}[4 + hnumUnselBp-1]$
		\State $\mathit{hnumUnselBp} \gets \mathit{hnumUnselBp} - 1$
		\State $\mathit{numUnselBp} \gets \mathit{numUnselBp} - 2$
		\Else
		\State $\mathit{bp}1 = \mathit{bp}[(int64)(\mathit{x}_{i}\times 10^{15})\mod \mathit{numUnselBp}]$
		\State Swap the values between $\mathit{bp}1$ and $\mathit{bp}[numUnselBp-1]$
		\State $\mathit{numUnselBp} \gets \mathit{numUnselBp} - 1$
		\State $\mathit{bp}2 = \mathit{bp}[(int64)(\mathit{x}_{i}\times 10^{15})\mod \mathit{numUnselBp}]$
		\State Swap the values between $\mathit{bp}2$ and $\mathit{bp}[numUnselBp-1]$
		\State $\mathit{numUnselBp} \gets \mathit{numUnselBp} - 1$
		\State $\mathit{hnumUnselBp} \gets \mathit{hnumUnselBp} - 1$
		\EndIf 
		\EndFunction
	\end{algorithmic}  
\end{algorithm}

Before selecting bit planes, we first pre-iterate Eq.(\ref{eqlogistic}) for $\mathit{T}_0$ times to avoid the harmful effect of the transitional procedure, 
where $T_0$ is a user-defined value. 
In our algorithm, we declare the data type of the state variables as double precision, 
which has a $15$-digit precision.
Then we quantize the generated values to get two bit planes $\mathit{bp}1$ and $\mathit{bp}2$.
The range of $\mathit{bp}1, \mathit{bp}2$ depends on the current encryption round $\mathit{permRnd}$. 
After the selection, we remove $\mathit{bp}1$ and $\mathit{bp}2$ from the array $\mathit{bps}$. 
Calling the Alg.~\ref{secbp} for four times in each round, we obtain four groups of bit planes to be scrambled. 


\subsection{Exchanging bits between two bit planes}
\label{sub2.2} 
A $256$-grayscale image of size $\mathit{M}\times \mathit{N}$ can be considered as a $3$-D bit matrix of size $\mathit{M}\times \mathit{N}\times 8$ in bit-level. 
It is represented as follows,
\begin{equation}
Img = 
\begin{pmatrix}
p_{00}^i& p_{01}^i & \cdots & p_{0\,N-1}^i\\ 
p_{10}^i&  p_{10}^i & \cdots & p_{1\,N-1}^i \\ 
\vdots &  \cdots&  \ddots & \vdots\\ 
p_{M-1\,0}^i&  p_{M-1\,1}^i&  \cdots& p_{M-1\,N-1}^i
\end{pmatrix},
\{i|0<=i<=7\}.
\label{bitmatrix}
\end{equation}
In bit-level permutation algorithms, calculating the bit positions in a $3$-D space is time-consuming.
To simplify the calculation, dimensionality reduction is performed on the $3$-D bit matrix.
We use BBD~\cite{zhou2014image} to decompose image data to obtain eight $2$-D bit planes.
Then each $2$-D bit plane converts to a $1$-D bit sequence .
The $\mathit{i}$-th $1$-D bit sequence is represented by,
\begin{equation}
bp^{i} = \{ b_0^i, b_1^i, b_2^i, ..., b_{M\times N - 1}^i\}.
\label{1dbs}
\end{equation} 

The detailed operation of exchanging bits between two bit planes is summarized in Alg.~\ref{PB2bp}. 
$(\mathit{bp^m},\mathit{bp^n})$ are two bit planes to be shuffled. 
$\mathit{lgInit_{exBit}}$ and $\mathit{lenBs}$ represent the initial value of logistic map used in bit exchanging and the length of the bit sequence converted from a bit plane, respectively. 
For each iteration, we extract a pseudo-random integer in range $[0, \mathit{lenBs}-1]$ from the current state of logistic map. 
Assuming that we get a value $\mathit{pos}$ after extraction, 
then we swap the values of current bit $\mathit{bp_i^m}$ and the target bit $\mathit{bp_{pos}^n}$. 
The outputs of Alg.~\ref{PB2bp} are two mutual permuted bit planes $\mathit{bpPerm^m}$ and $\mathit{bpPerm^n}$. 
Fig.~\ref{peredbp} shows the process of exchanging bits between two bit planes.

\begin{algorithm}[]  
	\caption{Exchanging bits between two bit planes.}  
	\label{PB2bp}  
	\begin{algorithmic}[1]  
		\Require  
		$\mathit{bp^m}, \mathit{bp^n}, \mathit{lgInit_{exBit}}, \mathit{lenBs}$
		\Ensure  
		$\mathit{bpPerm^m}, \mathit{bpPerm^n}$
		\Function{bpExchangebits}{$\mathit{bp^m},\mathit{bp^n}, \mathit{lgInit_{exBit}}, \mathit{lenBs}$}
		\State Initialize the bit position $\mathit{pos}$ to $0$
		\State $x_0 \gets \mathit{lgInit_{exBit}}$ 
		\State Preiterate logistic map for $\mathit{T}_0$ times
		\State $x_0 \gets \mathit{x_{T_0}}$
		\For{$\mathit{i} = 0$ to $\mathit{lenBs}-1$}
		\State Iterate the logistic map to generate a new value $x_i$
		\State $\mathit{pos} \gets (int64)(x_i \times 10^{15})\mod lenBs$
		\State swap the bit values between $\mathit{bp_i^m}$ and $\mathit{bp_{pos}^n}$
		\EndFor
		\State $\mathit{bpPerm^m} \gets \mathit{bp^m}$ and $\mathit{bpPerm^n} \gets \mathit{bp^n}$
		\EndFunction
	\end{algorithmic}  
\end{algorithm}
\begin{figure}[htbp]
	\centerline{\includegraphics[width = 0.9\textwidth]{permutationimg/perimg.jpg}}  
	\caption{Exchanging bits between two bit planes.} \label{peredbp}
\end{figure}

\subsection{The permutation process}
\label{effectper}
This section constructs the entire parallel permutation algorithm, as shown in Alg.~\ref{parallelper}. 
This algorithm needs to be run on a CPU with at least four threads.
As aforementioned, $\mathit{lgInit_{bpgrp}}$ is the initial value of the logistic map used in Alg.~\ref{secbp}.
Firstly, eight bit planes $\mathit{bps}$ are divided into four groups. 
Secondly, we create four threads and set their state to suspend as there are many thread-related parameters that need to be set before execution.
We set thread affinity to guarantee that each thread runs on different processors.
Then we set thread function parameters to make different threads smoothly perform the bits scrambling operation in each group.
For each thread, the logistic map used in exchanging needs to be assigned an initial value, which is denoted by $\mathit{lgInit}^k_\mathit{exBit}, k\in[0,3]$.
At last, the thread execution is resumed. 
Four groups shuffle bit planes in a parallel way. 
The multi-thread programming is implemented with the help of Windows API.
The outputs are eight shuffled bit planes $\mathit{bpPerms}$. 

\begin{algorithm}[] 
	\caption{The proposed parallel bit-level permutation.}  
	\label{parallelper}  
	\begin{algorithmic}[1]  
		\Require  
		$\mathit{lgInit_{bpgrp}}, (\mathit{lgInit}^k_\mathit{exBit},k\in[0, 3]), \mathit{permRnd}, \mathit{lenBs}, \mathit{bps}, \mathit{hnumUnselBp}, \mathit{numUnselBp}$
		\Ensure  
		$\mathit{bpPerms}$
		\Function{bpPermutation}{$\mathit{lgInit_{bpgrp}}, (\mathit{lgInit}^k_\mathit{exBit},k\in[0, 3]), \mathit{permRnd}, \mathit{bps}, \mathit{lenBs}$}
		\For{$\mathit{i} = 0$ to $3$}
		\State \Call{bpGrp}{$\mathit{lgInit_{bpgrp}}, \mathit{permRnd}, \mathit{bp}, \mathit{hnumUnselBp}, \mathit{numUnselBp}$}
		\EndFor
		\State Get four group of bit planes, $(\mathit{gbp}^k_1\leftrightarrow \mathit{gbp}^k_2) $
		\For{$\mathit{k} = 0$ to $3$}
		\State Create $\mathit{Thread^k}$ and suspend
		\State SetThreadPriority
		\State SetThreadAffinityMask
		\State Assign thread function and its argument
		\EndFor
		\State \textbf{spawn}
		\State Resume the execution of $\mathit{Thread^k}$ and \Call{bpExchangebits}{$\mathit{bp}^{\mathit{gbp}^k_1},\mathit{bp}^{\mathit{gbp}^k_2}, \mathit{lgInit}^k_\mathit{exBit}, \mathit{lenBs}$}
		\State \textbf{sync}
		\EndFunction
	\end{algorithmic}  
\end{algorithm}


\begin{figure}
	\begin{center}
		\subfigure[]{
			\label{figlena1}
			\includegraphics[width=0.25\linewidth]{permeffect/Lena.jpg}
		}
		\subfigure[]{
			\label{figlena2}
			\includegraphics[width=0.25\linewidth]{permeffect/pswap.jpg}
		}
		\subfigure[]{
			\label{figlena3}
			\includegraphics[width=0.25\linewidth]{permeffect/bitperm.jpg}
		}
		\subfigure[]{
			\label{figlena4}
			\includegraphics[width=0.25\linewidth]{permeffect/Lenaim.jpg}
		}
		\subfigure[]{
			\label{figlena5}
			\includegraphics[width=0.25\linewidth]{permeffect/swap.jpg}
		}
		\subfigure[]{
			\label{figlena6}
			\includegraphics[width=0.25\linewidth]{permeffect/1rp.jpg}
		}	
	\end{center}
	\caption{The histogram of the image after permutation. (a)-(c) are the plain-image, 
		the scrambled image obtained using three rounds of pixel swapping operation, 
		and our proposed algorithm, respectively. 
		Their corresponding histograms are shown in (d)-(f), respectively.}
	\label{fig5}
\end{figure}

To measure the scrambling effect, we carry out a histogram analysis, and the results are shown in Fig.~\ref{fig5}.  
Figs.~\ref{figlena1}-\ref{figlena3} show the plain-image, 
the permuted image obtained using three rounds of pixel swapping operation~\cite{song2020novel}, 
and our proposed algorithm, respectively and their corresponding histograms are shown in Figs.~\ref{figlena4}-\ref{figlena6}, respectively.
As can be seen from Fig.~\ref{fig5}, the histogram remains unchanged when the permutation is in pixel-level, while the histogram of the proposed algorithm is flatter.
This proves that our scheme can hide the statistical properties of images.

Tab.~\ref{pertime} lists the time required to execute three rounds of the proposed algorithm and the comparison algorithms.
The size of the test image is $512\times512$.
Fig.~\ref{fig5} and Tab.~\ref{pertime} show that our proposed parallel bit-level offers the best trade-off between permutation efficiency and effect.

\begin{table}[htbp]
	\centering
	\footnotesize
	\caption{The time consumption of permutation operation of different algorithms.}
	\begin{tabular}{ccccc}
		\hline
		& Our work & Ref.~\cite{Zhang2016Image}  & Ref.~\cite{song2020novel}   & Ref.~\cite{wang2019fast} \\ \hline
		Time(s) & $0.049$      & $0.183$ & $0.024$ & $0.030$ \\
		Type    & bit-level   &  bit-level    &    pixel-level   & pixel-level  \\ \hline
	\end{tabular}
	\label{pertime}
\end{table}

==> Security.tex <==
\section{Security analysis}
\label{sec5}
\subsection{Key space analysis}
The key of our proposed cryptosystem consists of three parts, 
the initial value of the logistic map used for bit planes grouping, the initial values of the four logistic maps for permutation, and initial values of the Lorenz system.
As aforementioned, the data type of all above variables is decalred as double precision, which offers $53$ bits precision.
Therefore, the total key space is $2^{53\times 7} = 2^{371}$, which is secure enough to resist the brute-force attack on a modern computer~\cite{alvarez2006some}.
\subsection{Statistical attack analysis}
\subsubsection{Frequency distribution of pixel values}
\label{fred}
%If the frequency distribution of pixel values remains the same after encryption, 
%then it's possible for an attacker to obtain some information about the plaintext by analyzing the frequency distribution.
A good cryptosystem should make the frequency distribution uniform after encryption.
We use histogram analysis to visualize the frequency distribution of pixel values.
Fig.~\ref{hist} shows the frequency distributions of plain-image and its corresponding cipher-image.
As can be seen from this figure, our scheme provides adequate randomization in frequency distribution of the pixel values in cipher-image.
%This means that it's difficult for an attacker to obtain information about the pixel distribution of plaintext from ciphertext.
\begin{figure}[]
	\centering
	\mbox{
		\subfigure[The plain-image and the histograms of three color channels.]{\includegraphics [width=0.48\linewidth]{analysis/lena_hist.jpg}}
	}
	\mbox{
		\subfigure[The cipher-image and the histograms of three color channels.]{\includegraphics [width=0.48\linewidth]{analysis/cipher_hist.jpg}}
	}
	\caption{The histograms of plain-image and cipher-image.}
	\label{hist}
\end{figure}

\subsubsection{Information entropy analysis}
\label{insen}
Information entropy, which is the average minimum number of bits needed to encode a string of symbols, 
is a quantitative measure of the randomness and unpredictability of information content. 
To calculate the information entropy, we have
\begin{equation}
H(S) =  -\sum_{i=1}^N P(S_i)\log_2^{P(S_i)}, \label{entropy}
\end{equation}
where $\mathit{S}$ is a random variable which has $\mathit{N}$ possible values ${\mathit{S}_0, \mathit{S}_1, ..., \mathit{S}_{N-1}}$, and $\mathit{P(S_i)}$ is the probability of $\mathit{S_i}$.
From Eq.(\ref{entropy}), it can be seen that information entropy of a random source emitting $N$ symbols is $\log_2^N$.
For instance, the information entropy of a random image with $256$ gray levels is $8$.
Therefore, the information entropy of a cipher-image should be as close as possible to $8$ to ensure that an attacker can not obtain any information about plain-image
by analyzing the frequency of certain characters' occurence.
Tab.~\ref{inforen} lists information entropy of the plain-images and their corresponding cipher-images.
We show that information entropy of cipher-images is very close to $8$, which means our algorithm successfully hide the statistical information of plain-image.

\begin{table}[]
	\centering
	\footnotesize
	\caption{The information entropy of plain-images and and their corresponding cipher-images.}
	\begin{tabular}{ccccc}
		\hline
		\multirow{2}{*}{Filename} & \multirow{2}{*}{Size} & \multirow{2}{*}{Type} & \multicolumn{2}{c}{Information entropy} \\ \cline{4-5} 
		&                       &                       & Plain-image        & Cipher-image       \\ \hline
		Lena                      & $512\times 512$       & Color                 & $7.532720$         & $7.999336$         \\
		Baboon                    & $512\times 512$       & Color                 & $7.679608$         & $7.999238$         \\
		Peppers                   & $512\times 512$       & Color                 & $7.565483$         & $7.999283$         \\
		Male                      & $1024\times 1024$     & Gray                  & $7.575793$         & $7.999829$         \\ \hline
	\end{tabular}
	\label{inforen}
\end{table}

\subsubsection{Correlation of adjacent pixels analysis}
\label{capa}
A pixel in a digital image is not independent of each other, 
it usually has a strong correlation with adjacent ones in either horizontal, vertical, and diagonal directions.
%It means in some areas of the image, there is liitle difference in pixel values.
Obviously, an effective cryptosystem should eliminate these correlations.
%One of the measures of the quality of encryption effect is whether the algorithm weakens the correlation of adjacent pixels.
%The weaker the correlation in cipher-image, the better the encryption effect and the higher the security.
To quantitatively explore the correlation between adjacent pixels in an image, 
we can randomly sample $5000$ pairs of adjacent pixels from it and use Eq.(\ref{corre}) to calculate the correlation coefficients $r_{xy}$.
\begin{equation}
r_{xy} = \frac {\frac{1}{N}\sum_{i=1}^N (x_i - \bar{x})(y_i-\bar{y})} {\sqrt{(\frac{1}{N}\sum_{i=1}^N (x_i - \bar{x})^2) (\frac{1}{N}\sum_{i=1}^N (y_i - \bar{y})^2)}}, \label{corre}
\end{equation}
where $x_i, y_i$ are the values of the i$th$ pair of adjacent pixels, $\bar{x} = \frac{1}{N} \sum_{i=1}^{N} x_i$, $\bar{y} = \frac{1}{N} \sum_{i=1}^{N} y_i$, and $N$ is the number of sampled pixel pairs. 
We calculate the correlation coefficients of three test images and their corresponding cipher-images, 
and the results are shown in Tab.~\ref{correlation}.
From this table we can see that there are strong correlations between adjacent pixels in the plain-images as their correlation coefficients are close to $1$.
As for the cipher-image, adjacent pixels are uncorrelated since the correlation coefficients are close to $0$.

To visually demonstrate this correlation, 
we plot the values of all the sampled pixels pairs $(x_i, y_i)$ in a scatter diagram. 
Figs.~\ref{rhor}-\ref{rdia} and~\ref{rchor}-\ref{rcdia} show the scatter diagrams for horizontally, 
vertically and diagonally adjacent pixels in the red channel of the ``Lena" test image and its corresponding cipher-image, respectively. 
It can be seen that most of the points in Figs.~\ref{rhor}-\ref{rdia} are clustered around the diagonal, 
showing there are strong correlations between adjacent pixels in the plain-image.
While the points in Figs.~\ref{rchor}-\ref{rcdia} are evenly distributed throughout the entire plane,
showing that there is practically no correlations between adjacent pixels in the cipher-image.
Similar results can be obtained for the other two color channels.

It can therefore be concluded from the results of the analysis carried out in Sec.~\ref{fred}-\ref{capa}
that our cryptosystem is robust against frequency analysis.

% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
	\centering
	\footnotesize
	\caption{Correlation coefficients for test images and their corresponding cipher-images.}
	\begin{tabular}{lcclllll}
		\hline
		\multicolumn{1}{c}{\multirow{2}{*}{Image}} & \multirow{2}{*}{Direction} & \multicolumn{3}{c}{Plain-image}                                                            & \multicolumn{3}{c}{Cipher-image}                                      \\ \cline{3-8} 
		\multicolumn{1}{c}{}                       &                            & R                            & \multicolumn{1}{c}{G}        & \multicolumn{1}{c}{B}        & \multicolumn{1}{c}{R} & \multicolumn{1}{c}{G} & \multicolumn{1}{c}{B} \\ \hline
		\multicolumn{1}{c}{Lena}                   & Horizontal                 & $0.989312$                     & \multicolumn{1}{c}{$0.981822$} & \multicolumn{1}{c}{$0.958012$} & \multicolumn{1}{r}{$-0.023050$}             & \multicolumn{1}{r}{$0.007344$}              & \multicolumn{1}{r}{$-0.029864$}             \\
		& Vertical                   & $0.978200$                     & \multicolumn{1}{c}{$0.968409$} & \multicolumn{1}{c}{$0.933531$} & \multicolumn{1}{r}{$0.004765$}              & \multicolumn{1}{r}{$-0.016220$}             & \multicolumn{1}{r}{$-0.002356$}             \\
		& Diagonal                   & $0.966425$                     & \multicolumn{1}{c}{$0.957546$} & \multicolumn{1}{c}{$0.923295$} & \multicolumn{1}{r}{$0.006422$}              & \multicolumn{1}{r}{$-0.012235$}             & \multicolumn{1}{r}{$-0.014490$}             \\
		\multicolumn{1}{c}{Baboon}                 & Horizontal                 & \multicolumn{1}{c}{$0.868475$} & $0.769258$                     & $0.889039$                     & \multicolumn{1}{r}{$-0.015995$}             & \multicolumn{1}{r}{$-0.001557$}             & \multicolumn{1}{r}{$0.004471$}              \\
		& Vertical                   & \multicolumn{1}{c}{$0.923147$} & $0.866631$                     & $0.907679$                     & \multicolumn{1}{r}{$0.000646$}              & \multicolumn{1}{r}{$0.003576$}              & \multicolumn{1}{r}{$0.029390$}              \\
		& Diagonal                   & \multicolumn{1}{c}{$0.858655$} & $0.746770$                     & $0.841463$                     & \multicolumn{1}{r}{$0.032847$}              & \multicolumn{1}{r}{$0.000137$}              & \multicolumn{1}{r}{$0.032149$}              \\
		Peppers                                    & Horizontal                 & $0.969083$                     & $0.981142$                     & $0.971482$                     & \multicolumn{1}{r}{$0.010863$}              & \multicolumn{1}{r}{$-0.019556$}             & \multicolumn{1}{r}{$0.014533$}              \\
		& Vertical                   & $0.962223$                     & $0.981469$                     & $0.963510$                     & \multicolumn{1}{r}{$0.005096$}              & \multicolumn{1}{r}{$0.014960$}              & \multicolumn{1}{r}{$-0.011490$}             \\
		& Diagonal                   & $0.955185$                     & $0.968332$                     & $0.947219$                     & \multicolumn{1}{r}{$0.010197$}              & \multicolumn{1}{r}{$0.007493$}              & \multicolumn{1}{r}{$-0.008847$}             \\ \hline
	\end{tabular}
	\label{correlation}
\end{table}

\begin{figure}[]
	\centering
	\mbox{
		\subfigure[]{\label{rhor} \includegraphics [width=0.3\linewidth]{analysis/rhor.jpg}}
		\subfigure[]{\label{rver} \includegraphics [width=0.3\linewidth]{analysis/rver.jpg}}
		\subfigure[]{\label{rdia} \includegraphics [width=0.3\linewidth]{analysis/rdia.jpg}}
	}
	\mbox{
		\subfigure[]{\label{rchor} \includegraphics [width=0.3\linewidth]{analysis/rchor.jpg}}
		\subfigure[]{\label{rcver} \includegraphics [width=0.3\linewidth]{analysis/rcver.jpg}}
		\subfigure[]{\label{rcdia} \includegraphics [width=0.3\linewidth]{analysis/rcdia.jpg}}
	}
	\caption{The scatter diagrams of ``Lena", (a)-(c) and (d)-(f) are scatter diagrams for horizontally, 
	vertically and diagonally adjacent pixels in the red channel of the test image and its corresponding cipher-image, respectively}
	\label{corr}
\end{figure}

\subsection{Differential attack}
Differential attack is a kind of chosen-plaintext attack.
Chosen-plaintext attack means that an attacker can choose arbitrary plaintexts to be encrypted and try to crack the cryptosystem.
In differential attack, an attacker uses the same key to encrypt a certain number of plain-images with little difference which can be constructed by the attacker.
The attacker compares the output cipher-images to find the design flaws in the cryptosystem,
then he may create an algorithm which would allow him to decrypt the cryptosystem. 
The differential attack is impractical, if the cyptosystem can produce the same number of completely different cipher-images. 

Two criteria, $\mathit{NPCR}$ (the number of pixel change rate) and $\mathit{UACI}$ (the unified average changing intensity) 
are used to evaluate the ability of the cryptosystem to resist differential attack.
$\mathit{NPCR}$ is defined by,
\begin{equation}
NPCR = \frac{\sum_{k}^{R,G,B}\sum_{i=1}^{W}\sum_{j=1}^{H}D(i, j)}{3\times W\times H}\times 100\%,
\label{npcr}
\end{equation}
where $(R, G, B)$, $\mathit{W}$ and $\mathit{H}$ represent the three color channels, and the width and height of the image, respectively.
And $\mathit{D(i ,j)}$ tells whether the values in the same position in two images $\mathit{C}_1$ and $\mathit{C}_2$ are the same. 
It is defined by,
\begin{equation}
D(i, j) =\left\{\begin{matrix}
0\quad if\;C_1(i, j) = C_2(i, j),\\ 
1\quad if\;C_1(i, j) \neq C_2(i, j).
\end{matrix}\right.
\end{equation}
For two random images with $256$ gray levels, the theoretical value of $NPCR$ is $99.609\%$.
The $\mathit{UACI}$ is defined by,
\begin{equation}
UACI = \frac{1}{3\times W\times H}\left[\sum_{k}^{R,G,B}\sum_{i=1}^{W}\sum_{j=1}^{H}\frac{\left|C_1(i, j)-C_2(i, j)\right|}{2^{L}-1}\right]\times 100\%,
\end{equation}
where $L$ is gray-level.
The theoretical value of $\mathit{UACI}$ is $33.464\%$ with $L = 256$.

Considering the worst scenario, we construct two plain-images that differ only by $1$-bit in a randomly selected pixel.
And we use the same key to encrypt the two plain-images, and calculate the $\mathit{NPCR}$ and $\mathit{UACI}$ of the two corresponding cipher-images.
The modification information of the test images and the the values of encryption keys are listed in Tab.~\ref{modified} and Tab.~\ref{initkey}.
As our algorithm is a parallel image encryption algorithm using intra bitplane scrambling, 
the comparable algorithms we choose include a bit-level encryption algorithm~\cite{xu2019a}, 
a parallel encryption algorithm~\cite{mozaffari2018parallel}, and a pixel-level encryption algorithm~\cite{alawida2019a}.
Tab.~\ref{npua} compares $\mathit{NPCR}$ and $\mathit{UACI}$ of the proposed algorithm with other state-of-the-art algorithms.
It shows that the $\mathit{NPCR}$ and $\mathit{UACI}$ of our algorithm are closer to the theoretical values than other algorithms, 
demonstrating better ability to resist differential attack.
The average values of $\mathit{NPCR}$ and $\mathit{UACI}$ of our algorithm are the average values of three test images.
And the average values of~\cite{alawida2019a} are the mean values of all test images.
Our algorithm uses three rounds of encryption to resist differential attack.

%列出三篇对比文献
\begin{table}[]
	\centering
	\footnotesize
	\caption{The modification information of the test images.}
	\begin{tabular}{clcccc}
		\hline
		\multicolumn{1}{l}{Image}   & \multicolumn{1}{c}{Type}  & Size             & \begin{tabular}[c]{@{}c@{}}Color\\ channel\end{tabular} & \begin{tabular}[c]{@{}c@{}}Pixel\\ coordinates\end{tabular} & \multicolumn{1}{l}{The change of value} \\ \hline
		Lena                        & \multicolumn{1}{c}{color} & $512\times512$   & blue                                                      & $(149, 452)$                                                & $210\rightarrow211$                                     \\
		baboon                      & color                     & $512\times512$   & red                                                       & \multicolumn{1}{c}{$(280, 332)$}                            & $99\rightarrow100$                                      \\
		male                        & color                     & $1024\times1024$ & blue                                                      & $(852, 507)$                                                & $100\rightarrow101$                                     \\ \hline
	\end{tabular}
	\label{modified}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
	\footnotesize
	\centering
	\caption{The keys used in permutation and diffusion stages.}
	\begin{tabular}{cclcccc}
		\hline
		\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Permutation\\ stage\end{tabular}} & \multicolumn{2}{c}{$\mathit{lgInit_{bpgrp}}$} & $\mathit{lgInit}^0_\mathit{exBit}$    & $\mathit{lgInit}^1_\mathit{exBit}$    & $\mathit{lgInit}^2_\mathit{exBit}$    & $\mathit{lgInit}^3_\mathit{exBit}$    \\
		& \multicolumn{2}{c}{$0.45367635654491$}  & $0.13489635765491$ & $0.43156483545677$ & $0.94561443184614$ & $0.63412476254234$ \\ \hline
		\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Diffusion\\ stage\end{tabular}}   & \multicolumn{2}{c}{$lx^0_0$}              & \multicolumn{2}{c}{$ly^0_0$}              & \multicolumn{2}{c}{$lz^0_0$}              \\
		& \multicolumn{2}{c}{$18.9675361237645$}  & \multicolumn{2}{c}{$10.8235829485923$}  & \multicolumn{2}{c}{$23.4534759901934$}  \\ \hline
	\end{tabular}
	\label{initkey}
\end{table}
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
	\centering
	\footnotesize
	\caption{The results of $\mathit{NPCR}$ and $\mathit{UACI}$ test for different algorithms.}
	\begin{tabular}{cccccc}
		\hline
		Image                                        & Test criteria & Our work  & Ref.~\cite{xu2019a}        & Ref.~\cite{mozaffari2018parallel}         & Ref.~\cite{alawida2019a}        \\ \hline
		\multirow{2}{*}{Lena}                        & $\mathit{NPCR}$        & $0.99602$ & $0.99618$ & $0.99580$ & $0.99620$ \\
		& $\mathit{UACI}$        & $0.33465$ & $0.33499$ & $0.33080$ & $0.33391$ \\
		\multirow{2}{*}{baboon}                      & $\mathit{NPCR}$        & $0.99617$ & \textemdash         & $0.99590$        & $0.99601$ \\
		& $\mathit{UACI}$        & $0.33492$ & \textemdash         & $0.31560$          & $0.33424$ \\
		\multirow{2}{*}{man}                         & $\mathit{NPCR}$        & $0.99606$ & \textemdash         & \textemdash & \textemdash         \\
		& $\mathit{UACI}$        & $0.33452$ & \textemdash         &\textemdash  & \textemdash         \\
		\multicolumn{1}{l}{\multirow{2}{*}{average}} & $\mathit{NPCR}$        & $0.99608$ & \textemdash         & \textemdash         & $0.99618$ \\
		\multicolumn{1}{l}{}                         & $\mathit{UACI}$        & $0.33470$ & \textemdash         & \textemdash       & $0.33496$ \\ \hline
	\end{tabular}
	\label{npua}
\end{table}

\begin{table}[htbp]
	\centering
	\footnotesize
	\caption{The test keys for key sensitivity analysis.}
	\begin{tabular}{ccccc}
		\hline
		Key No.   & the change of subkey   & key value                                                        & \multicolumn{1}{c}{Cipher-images} & \multicolumn{1}{l}{Differential images} \\ \hline
		$(1)$ & \textemdash     & \multicolumn{1}{l}{random-generated as shown in Tab.~\ref{initkey}} & Fig.\ref{c}                        & \multicolumn{1}{c}{\textemdash}     \\
		$(2)$ & $\mathit{lgInit_{bpgrp}}$ & $0.45367635654492$                                          & Fig.\ref{x0}                       & Fig.\ref{x0c}                        \\
		$(3)$ & $\mathit{lgInit}^0_\mathit{exBit}$   & $0.13489635765492$                                          & Fig.\ref{x1}                        & Fig.\ref{x1c}                        \\
		$(4)$ & $\mathit{lgInit}^1_\mathit{exBit}$   & $0.43156483545678$                                          & Fig.\ref{x2}                        & Fig.\ref{x2c}                        \\
		$(5)$ & $\mathit{lgInit}^2_\mathit{exBit}$   & $0.94561443184615$                                          & Fig.\ref{x3}                        & Fig.\ref{x3c}                        \\
		$(6)$ & $\mathit{lgInit}^3_\mathit{exBit}$   & $0.63412476254235$                                          & Fig.\ref{x4}                       & Fig.\ref{x4c}                        \\
		$(7)$ & $lx^0_0$     & $18.9675361237646$                                          & Fig.\ref{lx}                        & Fig.\ref{lxc}                        \\
		$(8)$ & $ly^0_0$     & $10.8235829485924$                                          & Fig.\ref{ly}                        & Fig.\ref{lyc}                        \\
		$(9)$ & $lz^0_0$     & $23.4534759901935$                                          & Fig.\ref{lz}                        & Fig.\ref{lzc}                        \\ \hline
	\end{tabular}
	\label{keysen}
\end{table}

\begin{figure}[]
	\centering
	\mbox{
		\subfigure[]{\label{lenna}\includegraphics [width=0.15\linewidth]{keysen/lenna.jpg}}
		\subfigure[]{\label{c} \includegraphics [width=0.15\linewidth]{keysen/c.jpg}}
		\subfigure[]{\label{x0} \includegraphics [width=0.15\linewidth]{keysen/x0.jpg}}
		\subfigure[]{\label{x1} \includegraphics [width=0.15\linewidth]{keysen/x1.jpg}}
		\subfigure[]{\label{x2} \includegraphics [width=0.15\linewidth]{keysen/x2.jpg}}
		\subfigure[]{\label{x3} \includegraphics [width=0.15\linewidth]{keysen/x3.jpg}}
	}
	\mbox{
		\subfigure[]{\label{x4} \includegraphics [width=0.15\linewidth]{keysen/x4.jpg}}
		\subfigure[]{\label{lx} \includegraphics [width=0.15\linewidth]{keysen/lx.jpg}}
		\subfigure[]{\label{ly} \includegraphics [width=0.15\linewidth]{keysen/ly.jpg}}
		\subfigure[]{\label{lz} \includegraphics [width=0.15\linewidth]{keysen/lz.jpg}}
		\subfigure[]{\label{x0c} \includegraphics [width=0.15\linewidth]{keysen/x0c.jpg}}
		\subfigure[]{\label{x1c} \includegraphics [width=0.15\linewidth]{keysen/x1c.jpg}}
	}
	\mbox{
		\subfigure[]{\label{x2c} \includegraphics [width=0.15\linewidth]{keysen/x2c.jpg}}
		\subfigure[]{\label{x3c} \includegraphics [width=0.15\linewidth]{keysen/x3c.jpg}}
		\subfigure[]{\label{x4c} \includegraphics [width=0.15\linewidth]{keysen/x4c.jpg}}
		\subfigure[]{\label{lxc} \includegraphics [width=0.15\linewidth]{keysen/lxc.jpg}}
		\subfigure[]{\label{lyc} \includegraphics [width=0.15\linewidth]{keysen/lyc.jpg}}
		\subfigure[]{\label{lzc} \includegraphics [width=0.15\linewidth]{keysen/lzc.jpg}}
	}
	\caption{Key sensitivity test in encryption process.}
	\label{keyen}
\end{figure}

\begin{figure}[]
	\centering
	\mbox{
		\subfigure[]{\label{de} \includegraphics [width=0.15\linewidth]{keyde/de.jpg}}
		\subfigure[]{\label{dex0} \includegraphics [width=0.15\linewidth]{keyde/dex0.jpg}}
		\subfigure[]{\label{dex1} \includegraphics [width=0.15\linewidth]{keyde/dex1.jpg}}
		\subfigure[]{\label{dex2} \includegraphics [width=0.15\linewidth]{keyde/dex2.jpg}}
	}
	\mbox{
		\subfigure[]{\label{dex3} \includegraphics [width=0.15\linewidth]{keyde/dex3.jpg}}
		\subfigure[]{\label{dex4} \includegraphics [width=0.15\linewidth]{keyde/dex4.jpg}}
		\subfigure[]{\label{dexlx} \includegraphics [width=0.15\linewidth]{keyde/delx.jpg}}
		\subfigure[]{\label{dexly} \includegraphics [width=0.15\linewidth]{keyde/dely.jpg}}
		\subfigure[]{\label{dexlz} \includegraphics [width=0.15\linewidth]{keyde/delz.jpg}}
	}
	
	\caption{Key sensitivity test in decryption process.}
	\label{keyde}
\end{figure}

\begin{table}[!htbp]
	\centering
	\footnotesize
	\caption{The encryption time of different algorithms.}
	\begin{tabular}{ccccc}
		\hline
		\multirow{2}{*}{The encryption algorithm} & \multirow{2}{*}{Number of encryption rounds} & \multicolumn{3}{c}{The encryption time(s) of different image size} \\ \cline{3-5} 
		&                                              & $256\times 256$      & $512\times 512$     & $1024\times 1024$     \\ \hline
		Our work                                  & $3$                                           & $0.035$              & $0.130$             & $0.571$               \\
		Ref.~\cite{xu2019a}                                         & $1$                                            & \textemdash                  & $0.107$             & \textemdash                   \\
		Ref.~\cite{mozaffari2018parallel}                                         & \textemdash                                            & $0.430$              & $1.100$             & $2.250$               \\
		Ref.~\cite{alawida2019a}                                         & $2$                                            & $0.621$              & \textemdash                 & \textemdash                   \\ \hline
	\end{tabular}
	\label{encryptionspeed}
\end{table}
\subsection{Key sensitivity analysis}
A cryptographic algorithm could be said to be sensitive to the key if it produces completely different ciphertexts when encrypting the same plaintext using different keys.
%We make tiny changes to keys to test the key sensitivity of our cryptosystem.
%In encryption process, if the user uses two sets of keys with a tiny difference to encrypt a same plain-image,
 %a big difference between two cipher-images should be produced.
The same is true for decryption process. 
That is, we can not obtain any information about the plaintext even if there is only a tiny difference between the decryption and encryption key.
%, in decryption phase, successful decryption can not be carried out when the wrong key is used.
\subsubsection{Encryption key sensitivity analysis}
To evaluate the key sensitivity of the encryption process,
we first generate a random secret key consisting of $8$ subkeys as the original key.
Then we construct $8$ different test keys, 
each of which differs only in the least significant bit of one subkey from the original key.
Finally, we encrypt a test image using the original and test keys and calculate the difference between their corresponding cipher-images.
For instance, we take the key listed in Tab.~\ref{initkey} as the original key, 
and the $8$ test keys generated from it are shown in Tab.~\ref{keysen}.
Figs.~\ref{lenna} shows the palin-image.
Its corresponding cipher-images encrypted using the original and test keys are shown in Figs.~\ref{c} and~\ref{x0}-\ref{lz}, respectively.
The differential images between the cipher-image obtained using the original key 
and each of the cipher-images obtained using the test keys are shown in Figs.~\ref{x0c}-\ref{lzc}, respectively.
%Tab. lists the key values after modifying the least significant bit, 
%the serial number of corresponding cipher-images and the corresponding differential images.
%Fig.~\ref{keyen} shows the plain-image, 
%the corresponding cipher-images and differential images using the keys listed in Tab.~\ref{initkey} and Tab.~\ref{keysen}.
As there are no continuous black pixels in each differential image, 
it indicates that the cipher-images are completely different even though only the least signigicant bit is changed of the encryption key, 
demonstrating good key sensitivity in encryption process.
\subsubsection{Decryption key sensitivity analysis}
We use Key No. $(1)-(9)$ to decrypt the cipher-image encrypted by Key No. $(1)$.
The corresponding decrypted images are shown in Figs.~\ref{de}-\ref{dexlz}, respectively.
It shows that the cipher-image can be correctly decrypted only under the correct key.

\subsection{Encryption speed analysis}
We compare the encryption speed of our proposed algorithm with the state-of-the-art works~\cite{xu2019a, mozaffari2018parallel, alawida2019a}.
The experiments run on a computer with Intel(R) Core(TM) i$7$-$6700$ CPU($4$ cores, $8$ threads) and $8$GB RAM.
The developing platform is codeblocks $20.03$.
The encryption time is listed in Tab.~\ref{encryptionspeed}.
Notably, the execution time of our algorithm consists of performing three rounds of encryption, 
while the encryption time of algorithm~\cite{xu2019a} does not include the time spent generating the three $3$D Latin cubes,
the number of encryption rounds of Ref.~\cite{mozaffari2018parallel} is not given the 
and the encryption time of algorithm~\cite{alawida2019a} consists of performing two rounds of encryption.
The encryption time of our proposed algorithm is the average time of $10$ test times, proving the high encryption efficiency.



